Black hole and galaxy co-evolution in radio-loud AGN at z ~ 0.3-4

There exists a well known relation between the mass of the supermassive black hole (SMBH) in the center of galaxies and their bulge mass or central velocity dispersion. This suggests a co-evolution between SMBH and their galaxy hosts. Our aim is to study this relation specifically for radio loud galaxies, and as a function of redshift $z$. We selected a sample of radio-galaxies and AGN by cross-matching the low radio frequency sources from VLA FIRST with spectroscopically confirmed sources from wide field surveys including SDSS DR14 ugriz and DES DR2 grzY in optical, WISE in infrared, and the Galaxy And Mass Assembly (GAMA) spectroscopic survey. Keeping only high signal to noise (S/N) sources in WISE magnitudes, and those with broad emission lines, we selected a sub sample of 42 radio sources, all with infrared-to-optical counterparts, for which we characterized the stellar, star formation, and black hole properties. We estimated the central SMBH mass, the stellar mass $M_\star$, the Eddington ratio $\eta$ and the jet power, $Q_{\rm jet}$. The relation between SMBH mass, $M_\star$, $\eta$ and $z$ are put into context by comparing them with scaling relations ($M_{\rm BH}$--$M_{\star}$, $M_{\rm BH}/M_\star$--$z$, $M_{\rm BH}$--$Q_{\rm jet}$ and $Q_{\rm jet}$--$\eta$) from the literature. An evolutionary scenario where radio-mode AGN feedback (or the cluster environments) regulate the accretion onto the SMBHs and the stellar mass assembly of the radio sources is discussed, which may explain the observed phenomenology, and in particular the presence of radio sources with high $M_{\rm BH}/M_\star$ ratios. This pilot study represents a benchmark for future ones using wide field surveys such as Euclid and the Vera Rubin telescope.

==> table_mass.tex <==
\begin{table}
\begin{tabular}{cccccccc}
$Survey$ & $RGid$ & $z$ & $Line$ & $FWHM$ & $L_{line}$ & $M_{BH}$ & $M_{\star}$ \\
deep & 16 & 1.22 & $M_{g}II$    & 4.08$ \pm $0.42 & 42.53$ \pm $41.71 & 8.0$ \pm $0.12 & 10.4 \\
deep & 49 & 0.88 & $H_{\beta}$  & 6.77$ \pm $0.11 & 44.02$ \pm $42.25 & 9.3$ \pm $0.04 & 11.95 \\
deep & 52 & 2.21 & $M_{g}II$    & 6.0$ \pm $0.43 & 43.41$ \pm $42.91 & 8.88$ \pm $0.13 & 11.73 \\
deep & 60 & 0.32 & $H_{\alpha}$ & 1.74$ \pm $0.07 & 41.88$ \pm $40.49 & 7.14$ \pm $0.04 & 10.54 \\
deep & 62 & 1.64 & $M_{g}II$    & 3.2$ \pm $0.11 & 43.26$ \pm $41.96 & 8.25$ \pm $0.08 & 11.02 \\
deep & 79 & 1.76 & $M_{g}II$    & 6.48$ \pm $0.16 & 43.47$ \pm $42.33 & 8.99$ \pm $0.08 & 11.48 \\
deep & 81 & 0.78 & $M_{g}II$    & 12.47$ \pm $2.07 & 42.14$ \pm $41.66 & 8.72$ \pm $0.18 & 10.76 \\
deep & 82 & 2.88 & $CIV$        & 5.26$ \pm $0.37 & 43.49$ \pm $42.92 & 8.73$ \pm $0.23 & 11.25 \\
deep & 83 & 0.68 & $H_{\beta}$  & 7.03$ \pm $1.67 & 41.87$ \pm $41.37 & 8.28$ \pm $0.23 & 11.11 \\
deep & 104 & 0.98 & $H_{\beta}$ & 6.31$ \pm $0.3 & 43.47$ \pm $42.34 & 8.97$ \pm $0.06 & 11.15 \\
deep & 113 & 2.08 & $M_{g}II$   & 5.89$ \pm $0.24 & 43.62$ \pm $42.72 & 9.0$ \pm $0.09 & 11.75 \\
deep & 151 & 2.6 & $M_{g}II$    & 7.68$ \pm $0.3 & 44.47$ \pm $43.73 & 9.76$ \pm $0.09 & 11.54 \\
deep & 159 & 1.08 & $M_{g}II$   & 3.95$ \pm $0.21 & 42.94$ \pm $41.7 & 8.22$ \pm $0.09 & 10.68 \\
deep & 177 & 0.47 & $H_{\beta}$ & 5.31$ \pm $0.14 & 42.6$ \pm $41.03 & 8.39$ \pm $0.06 & 10.45 \\
deep & 190 & 1.98 & $CIV$       & 14.66$ \pm $1.29 & 44.4$ \pm $43.76 & 10.04$ \pm $0.24 & 11.49 \\
deep & 195 & 0.36 & $H_{\beta}$ & 2.9$ \pm $0.03 & 42.42$ \pm $40.62 & 7.78$ \pm $0.06 & 10.94 \\
deep & 197 & 3.79 & $CIV$       & 1.93$ \pm $0.39 & 43.64$ \pm $42.93 & 7.92$ \pm $0.28 & 11.11 \\
deep & 205 & 1.68 & $M_{g}II$   & 7.22$ \pm $0.18 & 43.93$ \pm $42.68 & 9.38$ \pm $0.07 & 11.23 \\
deep & 206 & 1.15 & $M_{g}II$   & 4.12$ \pm $0.11 & 43.54$ \pm $42.02 & 8.64$ \pm $0.07 & 11.05 \\
deep & 214 & 0.77 & $H_{\beta}$ & 11.05$ \pm $0.48 & 43.42$ \pm $42.14 & 9.43$ \pm $0.06 & 10.43 \\
deep & 237 & 0.95 & $M_{g}II$   & 9.88$ \pm $0.99 & 43.24$ \pm $42.45 & 9.21$ \pm $0.12 & 10.27 \\
GAMA DR3 & 30401 & 0.35 & $H_{\alpha}$  & 1.19$ \pm $-0.0 & 42.38$ \pm $41.72 & 8.64$ \pm $0.0 & 11.14 \\
GAMA DR3 & 55673 & 0.44 & $H_{\beta}$   & 1.2$ \pm $0.19 & 41.66$ \pm $41.0 & 8.45$ \pm $0.03 & 11.19 \\
GAMA DR3 & 71277 & 0.32 & $H_{\alpha}$  & 1.05$ \pm $0.11 & 41.99$ \pm $41.08 & 8.36$ \pm $0.01 & 11.23 \\
GAMA DR3 & 165213 & 0.31 & $H_{\alpha}$ & 1.19$ \pm $-0.0 & 42.79$ \pm $40.89 & 8.82$ \pm $0.0 & 11.27 \\
GAMA DR3 & 196970 & 0.32 & $H_{\beta}$  & 1.2$ \pm $-0.0 & 40.89$ \pm $40.13 & 8.08$ \pm $0.01 & 11.08 \\
GAMA DR3 & 208794 & 0.45 & $H_{\beta}$  & 1.2$ \pm $-0.0 & 41.35$ \pm $40.32 & 8.3$ \pm $0.01 & 10.92 \\
GAMA DR3 & 249591 & 0.43 & $H_{\beta}$  & 1.2$ \pm $-0.0 & 41.66$ \pm $41.15 & 8.45$ \pm $0.01 & 11.31 \\
GAMA DR3 & 251343 & 0.76 & $H_{\beta}$  & 1.19$ \pm $-0.0 & 43.96$ \pm $42.58 & 9.57$ \pm $0.0 & 11.54 \\
GAMA DR3 & 298359 & 0.34 & $H_{\alpha}$ & 1.19$ \pm $-0.0 & 42.07$ \pm $41.21 & 8.51$ \pm $0.0 & 10.92 \\
GAMA DR3 & 319591 & 0.56 & $H_{\beta}$  & 1.2$ \pm $-0.0 & 41.64$ \pm $40.55 & 8.43$ \pm $0.01 & 11.28 \\
GAMA DR3 & 372455 & 0.31 & $H_{\alpha}$ & 1.19$ \pm $-0.0 & 42.66$ \pm $41.9 & 8.77$ \pm $0.0 & 11.02 \\
GAMA DR3 & 537618 & 0.49 & $H_{\beta}$  & 1.1$ \pm $0.04 & 43.86$ \pm $42.62 & 9.45$ \pm $0.0 & 10.79 \\
GAMA DR3 & 618703 & 0.6 & $H_{\beta}$   & 1.2$ \pm $-0.0 & 43.61$ \pm $42.41 & 9.4$ \pm $0.0 & 11.41 \\
GAMA DR3 & 714133 & 0.56 & $H_{\beta}$  & 1.2$ \pm $-0.0 & 42.25$ \pm $40.69 & 8.74$ \pm $0.0 & 10.8 \\
GAMA DR3 & 714228 & 0.34 & $H_{\beta}$  & 1.2$ \pm $-0.0 & 40.86$ \pm $40.03 & 8.06$ \pm $0.01 & 10.67 \\
GAMA DR3 & 720847 & 0.42 & $H_{\beta}$  & 1.19$ \pm $-0.0 & 41.92$ \pm $40.53 & 8.57$ \pm $0.01 & 11.11 \\
GAMA DR3 & 721940 & 0.64 & $H_{\beta}$  & 1.2$ \pm $-0.0 & 43.31$ \pm $42.28 & 9.25$ \pm $0.0 & 10.94 \\
GAMA DR3 & 745066 & 0.38 & $H_{\beta}$  & 1.19$ \pm $-0.0 & 41.73$ \pm $40.32 & 8.47$ \pm $0.01 & 11.72 \\
GAMA DR3 & 746605 & 0.37 & $H_{\beta}$  & 1.24$ \pm $0.09 & 43.37$ \pm $42.37 & 9.31$ \pm $0.01 & 10.7 \\
GAMA DR3 & 748144 & 0.59 & $H_{\beta}$  & 1.22$ \pm $-0.0 & 43.08$ \pm $42.39 & 9.16$ \pm $0.0 & 11.67 \\
GAMA DR3 & 748815 & 0.33 & $H_{\beta}$  & 1.19$ \pm $-0.0 & 42.05$ \pm $40.34 & 8.63$ \pm $0.01 & 10.87 \\
GAMA DR3 & 804203 & 0.51 & $H_{\beta}$  & 1.2$ \pm $-0.0 & 41.44$ \pm $40.83 & 8.34$ \pm $0.01 & 10.79 \\
GAMA DR3 & 835899 & 0.76 & $H_{\beta}$  & 1.19$ \pm $-0.0 & 42.24$ \pm $40.88 & 8.72$ \pm $0.0 & 11.83 \\
GAMA DR3 & 887308 & 0.55 & $H_{\beta}$  & 1.2$ \pm $-0.0 & 43.17$ \pm $42.05 & 9.18$ \pm $0.0 & 11.55 \\
\end{tabular}
\end{table}


==> table_props.tex <==
\begin{table}
\begin{tabular}{ccccccccc}
$Survey$ & $RGid$ & $z$ & $Line$ & $M_{BH}$ & $L_{blr}$ & $L_{edd}$ & $eta$ & $Q_{jet}$ \\
deep & 16 & 1.22 & $M_{g}II$ & 8.0$ \pm $0.12 & 43.5 & 46.1 & -1.6 & 45.81 \\
deep & 49 & 0.88 & $H_{\beta}$ & 9.3$ \pm $0.04 & 45.06 & 47.4 & -1.34 & 45.69 \\
deep & 52 & 2.21 & $M_{g}II$ & 8.88$ \pm $0.13 & 44.51 & 46.99 & -1.48 & 44.94 \\
deep & 60 & 0.32 & $H_{\alpha}$ & 7.14$ \pm $0.04 & 42.44 & 45.24 & -1.8 & 43.22 \\
deep & 62 & 1.64 & $M_{g}II$ & 8.25$ \pm $0.08 & 44.27 & 46.35 & -1.07 & 44.9 \\
deep & 79 & 1.76 & $M_{g}II$ & 8.99$ \pm $0.08 & 44.73 & 47.09 & -1.36 & 46.65 \\
deep & 81 & 0.78 & $M_{g}II$ & 8.72$ \pm $0.18 & 43.3 & 46.82 & -2.52 & 44.64 \\
deep & 82 & 2.88 & $CIV$ & 8.73$ \pm $0.23 & 44.28 & 46.83 & -1.55 & 45.83 \\
deep & 83 & 0.68 & $H_{\beta}$ & 8.28$ \pm $0.23 & 40.57 & 46.38 & -4.8 & 45.76 \\
deep & 104 & 0.98 & $H_{\beta}$ & 8.97$ \pm $0.06 & 44.56 & 47.07 & -1.52 & 44.66 \\
deep & 113 & 2.08 & $M_{g}II$ & 9.0$ \pm $0.09 & 44.67 & 47.1 & -1.43 & 45.1 \\
deep & 151 & 2.6 & $M_{g}II$ & 9.76$ \pm $0.09 & 45.13 & 47.86 & -1.73 & 44.75 \\
deep & 159 & 1.08 & $M_{g}II$ & 8.22$ \pm $0.09 & 43.95 & 46.32 & -1.37 & 46.21 \\
deep & 177 & 0.47 & $H_{\beta}$ & 8.39$ \pm $0.06 & 43.65 & 46.49 & -1.84 & 44.22 \\
deep & 190 & 1.98 & $CIV$ & 10.04$ \pm $0.24 & 45.05 & 48.14 & -2.08 & 46.05 \\
deep & 195 & 0.36 & $H_{\beta}$ & 7.78$ \pm $0.06 & 43.89 & 45.88 & -0.99 & 43.4 \\
deep & 197 & 3.79 & $CIV$ & 7.92$ \pm $0.28 & 44.43 & 46.02 & -0.59 & 45.61 \\
deep & 205 & 1.68 & $M_{g}II$ & 9.38$ \pm $0.07 & 45.19 & 47.48 & -1.29 & 45.28 \\
deep & 206 & 1.15 & $M_{g}II$ & 8.64$ \pm $0.07 & 44.58 & 46.74 & -1.16 & 45.66 \\
deep & 214 & 0.77 & $H_{\beta}$ & 9.43$ \pm $0.06 & 44.36 & 47.53 & -2.17 & 44.96 \\
deep & 237 & 0.95 & $M_{g}II$ & 9.21$ \pm $0.12 & 44.3 & 47.31 & -2.01 & 44.07 \\
GAMA DR3 & 30401 & 0.35 & $H_{\alpha}$ & 8.64$ \pm $0.0 & 34.01 & 46.74 & -2.73 & 44.02 \\
GAMA DR3 & 55673 & 0.44 & $H_{\beta}$ & 8.45$ \pm $0.03 & 33.91 & 46.55 & -2.64 & 43.51 \\
GAMA DR3 & 71277 & 0.32 & $H_{\alpha}$ & 8.36$ \pm $0.01 & 33.61 & 46.46 & -2.85 & 43.35 \\
GAMA DR3 & 165213 & 0.31 & $H_{\alpha}$ & 8.82$ \pm $0.0 & 34.45 & 46.92 & -2.47 & 42.99 \\
GAMA DR3 & 196970 & 0.32 & $H_{\beta}$ & 8.08$ \pm $0.01 & 32.74 & 46.18 & -3.44 & 43.11 \\
GAMA DR3 & 208794 & 0.45 & $H_{\beta}$ & 8.3$ \pm $0.01 & 33.6 & 46.4 & -2.8 & 43.26 \\
GAMA DR3 & 249591 & 0.43 & $H_{\beta}$ & 8.45$ \pm $0.01 & 33.91 & 46.55 & -2.64 & 43.75 \\
GAMA DR3 & 251343 & 0.76 & $H_{\beta}$ & 9.57$ \pm $0.0 & 36.21 & 47.67 & -1.46 & 44.42 \\
GAMA DR3 & 298359 & 0.34 & $H_{\alpha}$ & 8.51$ \pm $0.0 & 33.76 & 46.61 & -2.85 & 44.93 \\
GAMA DR3 & 319591 & 0.56 & $H_{\beta}$ & 8.43$ \pm $0.01 & 33.89 & 46.53 & -2.65 & 44.57 \\
GAMA DR3 & 372455 & 0.31 & $H_{\alpha}$ & 8.77$ \pm $0.0 & 34.29 & 46.87 & -2.58 & 43.67 \\
GAMA DR3 & 537618 & 0.49 & $H_{\beta}$ & 9.45$ \pm $0.0 & 36.11 & 47.55 & -1.44 & 43.96 \\
GAMA DR3 & 618703 & 0.6 & $H_{\beta}$ & 9.4$ \pm $0.0 & 35.86 & 47.5 & -1.64 & 44.11 \\
GAMA DR3 & 714133 & 0.56 & $H_{\beta}$ & 8.74$ \pm $0.0 & 34.5 & 46.84 & -2.34 & 43.99 \\
GAMA DR3 & 714228 & 0.34 & $H_{\beta}$ & 8.06$ \pm $0.01 & 33.11 & 46.16 & -3.05 & 44.11 \\
GAMA DR3 & 720847 & 0.42 & $H_{\beta}$ & 8.57$ \pm $0.01 & 34.17 & 46.67 & -2.5 & 44.07 \\
GAMA DR3 & 721940 & 0.64 & $H_{\beta}$ & 9.25$ \pm $0.0 & 35.56 & 47.35 & -1.79 & 44.26 \\
GAMA DR3 & 745066 & 0.38 & $H_{\beta}$ & 8.47$ \pm $0.01 & 33.77 & 46.57 & -2.8 & 43.3 \\
GAMA DR3 & 746605 & 0.37 & $H_{\beta}$ & 9.31$ \pm $0.01 & 35.62 & 47.41 & -1.79 & 43.03 \\
GAMA DR3 & 748144 & 0.59 & $H_{\beta}$ & 9.16$ \pm $0.0 & 35.33 & 47.26 & -1.93 & 43.95 \\
GAMA DR3 & 748815 & 0.33 & $H_{\beta}$ & 8.63$ \pm $0.01 & 33.94 & 46.73 & -2.79 & 44.68 \\
GAMA DR3 & 804203 & 0.51 & $H_{\beta}$ & 8.34$ \pm $0.01 & 33.69 & 46.44 & -2.75 & 43.82 \\
GAMA DR3 & 835899 & 0.76 & $H_{\beta}$ & 8.72$ \pm $0.0 & 34.49 & 46.82 & -2.33 & 43.9 \\
GAMA DR3 & 887308 & 0.55 & $H_{\beta}$ & 9.18$ \pm $0.0 & 35.42 & 47.29 & -1.87 & 43.8 \\
\end{tabular}
\end{table}

